DDRF: Denoising Diffusion Model for Remote Sensing Image Fusion

Denosing diffusion model, as a generative model, has received a lot of attention in the field of image generation recently, thanks to its powerful generation capability. However, diffusion models have not yet received sufficient research in the field of image fusion. In this article, we introduce diffusion model to the image fusion field, treating the image fusion task as image-to-image translation and designing two different conditional injection modulation modules (i.e., style transfer modulation and wavelet modulation) to inject coarse-grained style information and fine-grained high-frequency and low-frequency information into the diffusion UNet, thereby generating fused images. In addition, we also discussed the residual learning and the selection of training objectives of the diffusion model in the image fusion task. Extensive experimental results based on quantitative and qualitative assessments compared with benchmarks demonstrates state-of-the-art results and good generalization performance in image fusion tasks. Finally, it is hoped that our method can inspire other works and gain insight into this field to better apply the diffusion model to image fusion tasks. Code shall be released for better reproducibility.

==> sections/tabs.tex <==
%%%%%%%%%%%%%%%%%%%UNUSED WV3%%%%%%%%%%%%%%%%%%%%
%% reduce
\begin{table}[!htbp]
\caption{Result of quantitative metrics on reduced WV3 dataset.  Some conventional methods(the first 3 rows),  DL-based methods are compared. The best results are in boldface and the second results are in underline.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
method          & SAM($\pm$ std) &ERGAS($\pm$ std) & Q8($\pm$ std) & SCC($\pm$ std) \\ \hline \hline
BT-H            & 4.8985$\pm$1.3028 & 4.5150$\pm$1.3315 & 0.8182$\pm$0.1019 & 0.9240$\pm$0.0243 \\
BDSD-PC         & 5.4675$\pm$1.7185 & 4.6549$\pm$1.4667 & 0.8117$\pm$0.1063 & 0.9049$\pm$0.0419  \\ 
MTF-GLP-FS      & 5.3233$\pm$1.6548 & 4.6452$\pm$1.4441 & 0.8177$\pm$0.1014 & 0.8984$\pm$0.0466 \\ \hline
PNN             & 3.6798$\pm$0.7625 & 2.6819$\pm$0.6475 & 0.8929$\pm$0.0923 & 0.9761$\pm$0.0075  \\
PanNet          & 3.6156$\pm$0.7665 & 2.6660$\pm$0.6887 & 0.8906$\pm$0.0934 & 0.9757$\pm$0.0088 \\
DICNN           & 3.5929$\pm$0.7623 & 2.6733$\pm$0.6627 & 0.9004$\pm$0.0871 & 0.9763$\pm$0.0072 \\
MSDCNN          & 3.7773$\pm$0.8032 & 2.7608$\pm$0.6884 & 0.8900$\pm$0.0900 & 0.9741$\pm$0.0076 \\
FusionNet       & 3.3252$\pm$0.6978 & 2.4666$\pm$0.6446 & 0.9044$\pm$0.0904 & 0.9807$\pm$0.0069 \\
LAGNet          & 3.1042$\pm$0.5585 & 2.2999$\pm$0.6128 & 0.9098$\pm$0.0907 & 0.9838$\pm$0.0068 \\
DCFNet          & \ul{3.0264$\pm$0.7397} & \ul{2.1588$\pm$0.4563} & \ul{0.9051$\pm$0.0881} & \ul{0.9861$\pm$0.0038} \\ \hline
DDRF(ours)  & \textbf{2.7722$\pm$0.5112} & \textbf{2.0484$\pm$0.4500} & \textbf{0.9191$\pm$0.0824} & \textbf{0.9877$\pm$0.0033}  \\ \hline
Ideal value    & \textbf{0}   & \textbf{0}  & \textbf{1}  & \textbf{1} \\ \hline
\end{tabular}}
\hspace{2pt}
\label{table:wv3_reduce}
\end{table}

%% full
\begin{table}[!htbp]
\caption{Result of quantitative metrics on WV3 dataset with full-resolution. Some conventional methods, DL-based methods are compared. The best results are in boldface and the second results are in underline.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
method          &$D_\lambda$($\pm$std) &$D_s$($\pm$std) & QNR($\pm$std) \\ \hline \hline
BT-H            & 0.0574$\pm$0.0232 & 0.0810$\pm$0.0374 & 0.8670$\pm$0.0540 \\
BDSD-PC         & 0.0625$\pm$0.0235 & 0.0730$\pm$0.0356 & 0.8698$\pm$0.0531 \\ 
MTF-GLP-FS      & 0.0206$\pm$0.0082	& 0.0630$\pm$0.0284 & 0.9180$\pm$0.0346 \\ 
TV              & 0.0234$\pm$0.0061	& 0.0393$\pm$0.0227 & 0.9383$\pm$0.0269 \\ \hline
PNN             & \ul{0.0213$\pm$0.0080}	& 0.0428$\pm$0.0147 & 0.9369$\pm$0.0212 \\
PanNet          & \textbf{0.0165$\pm$0.0074}	& 0.0470$\pm$0.0213	& \ul{0.9374$\pm$0.0271} \\
DiCNN           & 0.0362$\pm$0.0111	& 0.0462$\pm$0.0175  & 0.9195$\pm$0.0258 \\
MSDCNN          & 0.0230$\pm$0.0091	& 0.0467$\pm$0.0199	& 0.9316$\pm$0.0271 \\
BDPN            & 0.0364$\pm$0.0142	&0.0459$\pm$0.0192	&0.9196$\pm$0.0308 \\
FusionNet       & 0.0239$\pm$0.0090	& \textbf{0.0364$\pm$0.0137}	&\textbf{0.9406$\pm$0.0197} \\
LAGNet          & 0.0368$\pm$0.0148	& \ul{0.0418$\pm$0.0152}	&0.9230$\pm$0.0247 \\
DCFNet          & 0.0781$\pm$0.0812 & 0.0508$\pm$0.0342 & 0.8771$\pm$0.1005 \\ \hline
DDRF(ours)  & 0.0741$\pm$0.0628 & 0.0586$\pm$0.0282 & 0.8715$\pm$0.0630 \\ \hline
Ideal value    & \textbf{0}   & \textbf{0}  & \textbf{1} \\ \hline
\end{tabular}}
\label{table:wv3_full}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%UNUSED GF2%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htbp]
\caption{Result of quantitative metrics on reduced GF2 dataset. Some conventional methods, CNN and transformer methods are compared.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
method         & SAM($\pm$ std) &ERGAS($\pm$ std) & Q4($\pm$ std) & SCC($\pm$ std) \\ \hline \hline
BT-H            & 1.6810$\pm$0.3168 & 1.5524$\pm$0.3642 & 0.9089$\pm$0.0292 & 0.9508$\pm$0.0150  \\
BDSD-PC         & 1.7110$\pm$0.3210 & 1.7025$\pm$0.4056 & 0.9932$\pm$0.0308 & 0.9448$\pm$0.0166  \\ 
MTF-GLP-FS     & 1.6757$\pm$0.3457 & 1.6023$\pm$0.3545 & 0.8914$\pm$0.0256 & 0.9390$\pm$0.0197 \\ \hline
PNN            & 1.0477$\pm$0.2264 & 1.0572$\pm$0.2355 & 0.9604$\pm$0.0100   & 0.9772$\pm$0.0054  \\
PanNet          & 0.9967$\pm$0.2119 & 0.9192$\pm$0.1906 & 0.9671$\pm$0.0099   & 0.9829$\pm$0.0035 \\
DICNN          & 1.0525$\pm$0.2310 & 1.0812$\pm$0.2510 & 0.9594$\pm$0.0101    & 0.9771$\pm$0.0058 \\
MSDCNN         & 1.0472$\pm$0.2210 & 1.0413$\pm$0.2309 & 0.9612$\pm$0.0108    & 0.9782$\pm$0.0050 \\
FusionNet      &  0.9735$\pm$0.2117    & 0.9878$\pm$0.2222   & 0.9641$\pm$0.0093 & 0.9806$\pm$0.0049 \\
LAGNet          & \ul{0.7859$\pm$0.1478}     & \ul{0.6869$\pm$0.1125}    & \ul{0.9804$\pm$0.0085} & \textbf{0.9906$\pm$0.0019} \\
DCFNet          & 0.8896$\pm$0.1577     & 0.8061$\pm$0.1369   & 0.9727$\pm$0.0100 & 0.9853$\pm$0.0024 \\ \hline
DDRF(ours)  & \textbf{0.6408$\pm$0.1203} & \textbf{0.5668$\pm$0.1010} & \textbf{0.9855$\pm$0.0078} & \ul{0.9859$\pm$0.0035} \\ \hline
Ideal value    & \textbf{0}   & \textbf{0}  & \textbf{1}  & \textbf{1} \\ \hline
\end{tabular}}
\label{table:gf2_reduce}
\end{table}

\begin{table}[!htbp]
\caption{Result of quantitative metrics on GF2 dataset with full-resolution. Some conventional methods, CNN and transformer methods are compared.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
method      &$D_\lambda$($\pm$ std) &$D_s$($\pm$ std) & QNR($\pm$ std) \\ \hline \hline
BT-H	    &0.0602$\pm$0.0252	&0.1313$\pm$0.0193	&0.8165$\pm$0.0305 \\
BDSD-PC 	&0.0759$\pm$0.0301	&0.1548$\pm$0.0280	&0.7812$\pm$0.0409 \\
MTF-GLP-FS	&0.0336$\pm$0.0129	&0.1404$\pm$0.0277	&0.8309$\pm$0.0334 \\
TV	        &0.0553$\pm$0.0422	&0.1118$\pm$0.0226	&0.8392$\pm$0.0531 \\ \hline
PNN	        &0.0367$\pm$0.0291	&0.0943$\pm$0.0224	&0.8726$\pm$0.0373 \\
PanNet	    &0.0206$\pm$0.0112	&0.0799$\pm$0.0178	&0.9011$\pm$0.0203 \\
DiCNN	    &0.0413$\pm$0.0128	&0.0992$\pm$0.0131	&0.8636$\pm$0.0165 \\
MSDCNN	    &0.0269$\pm$0.0131	&0.0730$\pm$0.0093	&0.9020$\pm$0.0128 \\
BDPN	    &0.0365$\pm$0.0225	&0.0765$\pm$0.0199	&0.8897$\pm$0.0257 \\
FusionNet	&0.0400$\pm$0.0126	&0.1013$\pm$0.0134	&0.8628$\pm$0.0184 \\
LAGConv	    &0.0324$\pm$0.0130	&0.0792$\pm$0.0136	&0.8910$\pm$0.0204 \\
DCFNet          &       &    &  \\ \hline
DDRF(ours)  & \textbf{0.0201$\pm$0.0109} & \textbf{0.0408$\pm$0.0103} & \textbf{0.9398$\pm$0.0137} \\ \hline
Ideal value    & \textbf{0}   & \textbf{0}  & \textbf{1} \\ \hline
\end{tabular}}
\label{table: gf2_full}
\end{table}

%%%%%%%%%%%%%%%%%%%%UNUSED QB%%%%%%%%%%%%%%%%%%%
\begin{table}[!ht]
\caption{Result of quantitative metrics on reduced QB dataset. Some conventional methods, CNN and transformer methods are compared.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
method          & SAM($\pm$ std) &ERGAS($\pm$ std) & Q4($\pm$ std) & SCC($\pm$ std) \\ \hline \hline
BDSD-PC         & 8.2620$\pm$2.0497 & 7.5420$\pm$0.8138 & 0.8323$\pm$0.1013 & 0.9030$\pm$0.0181 \\ 
MTF-GLP-FS      & 8.1131$\pm$1.9553 & 7.5102$\pm$0.7926 & 0.8296$\pm$0.0905 & 0.8998$\pm$0.0196 \\
BT-H            & 7.1943$\pm$1.5523 & 7.4008$\pm$0.8378 & 0.8326$\pm$0.0880 & 0.9156$\pm$0.0152 \\\hline
PNN             & 5.2054$\pm$0.9625 & 4.4722$\pm$0.3734 & 0.9180$\pm$0.0938 & 0.9711$\pm$0.0123 \\
PanNet          & 5.7909$\pm$1.1839 & 5.8629$\pm$0.8883 & 0.8850$\pm$0.0917 & 0.9485$\pm$0.0170 \\
DICNN           & 5.3795$\pm$1.0266 & 5.1354$\pm$0.4876 & 0.9042$\pm$0.0942 & 0.9621$\pm$0.0133 \\
FusionNet       & 4.9226$\pm$0.9077 & 4.1594$\pm$0.3212 & 0.9252$\pm$0.0902 & 0.9755$\pm$0.0104 \\
LAGNet          & 4.5473$\pm$0.8296 & \ul{3.8259$\pm$0.4196} & \ul{0.9335$\pm$0.0878} & \ul{0.9807$\pm$0.0091} \\
DCFNet          & \ul{4.5383$\pm$0.7397} & 3.8315$\pm$0.2915 & 0.9325$\pm$0.0903 & 0.9741$\pm$0.0101 \\ \hline
DDRF(ours)  & \textbf{4.3529$\pm$0.7319} & \textbf{3.5659$\pm$0.2845} & \textbf{0.9380$\pm$0.0896} & \textbf{0.9838$\pm$0.0073} \\ \hline
Ideal value    & \textbf{0}   & \textbf{0}  & \textbf{1} & \textbf{1} \\ \hline
\end{tabular}}
\label{table:qb_reduce}
\end{table}

\begin{table}[!htbp]
\caption{Result of quantitative metrics on QB dataset with full-resolution. Some conventional methods, CNN and transformer methods are compared.}
\label{tab: qb_full}
% \resizebox{\linewidth}{!}{
\begin{tabular}{l|cccc}
\hline
method          & $D_\lambda$($\pm$ std) &$D_s$($\pm$ std) & QNR($\pm$ std) \\ \hline \hline
BT-H            & 0.2300$\pm$0.0718	&0.1648$\pm$0.0167	&0.6434$\pm$0.0645   \\
BDSD-PC         & 0.1975$\pm$0.0334	&0.1636$\pm$0.0483	&0.6722$\pm$0.0577   \\ 
MTF-GLP-FS      & 0.0489$\pm$0.0149	&0.1383$\pm$0.0238	&0.8199$\pm$0.0340 \\ 
TV              & 0.0550$\pm$0.0142	&0.1009$\pm$0.0265	&0.8501$\pm$0.0365 \\ \hline

PNN             & 0.0569$\pm$0.0112	&0.0624$\pm$0.0239	&0.8844$\pm$0.0304  \\
PanNet          & \textbf{0.0410$\pm$0.0108}	&0.1137$\pm$0.0323	&0.8502$\pm$0.0390  \\
DiCNN           & 0.0920$\pm$0.0143	&0.1067$\pm$0.0210	&0.8114$\pm$0.0310 \\
MSDCNN	        & 0.0592$\pm$0.0152	&0.0667$\pm$0.0289	&0.8784$\pm$0.0390 \\
BDPN	        & 0.0739$\pm$0.0386	&\textbf{0.0492$\pm$0.0129}	&\ul{0.8807$\pm$0.0428} \\
FusionNet	    &\ul{0.0586$\pm$0.0189}	&\ul{0.0522$\pm$0.0088}	&\textbf{0.8922$\pm$0.0219} \\
LAGConv	        &0.0844$\pm$0.0238	&0.0676$\pm$0.0136	&0.8536$\pm$0.0178 \\
DCFNet          & & & \\ \hline
DDRF(ours) &0.1025$\pm$0.0266 &0.0552$\pm$0.0228 &0.8484$\pm$0.0416 \\ \hline
Ideal value    & \textbf{0}   & \textbf{0}  & \textbf{1} \\ \hline
\end{tabular}
% }
\end{table}

%%%%%%%%%%%%%%%%%UNUSED WV2%%%%%%%%%%%%%%%%%%%
\begin{table}[!htbp]
\centering
\caption{Generalization ability comparisons on WV2 reduced dataset.}
\label{tab: wv2_generalization}
\resizebox{\linewidth}{!}{
    \begin{tabular}{l|cccc}
    \hline
     method    &  SAM($\pm$ std) & ERGAS($\pm$ std) & Q8($\pm$ std) & SCC($\pm$ std)\\
     \hline \hline
     PNN &7.1158$\pm$1.6812& 5.6152$\pm$0.9431& 0.7619$\pm$0.0928&0.8782$\pm$0.0175\\
     PanNet &\ul{5.4948$\pm$0.7126} & \textbf{4.3371$\pm$0.5197}& \textbf{0.8401$\pm$0.0796}& \textbf{0.9177$\pm$0.0081}\\
     DiCNN &6.9216$\pm$0.7898 &6.2507$\pm$0.5745 &0.7205$\pm$0.0746 &0.8552$\pm$0.0289\\
     MSDCNN &6.0064$\pm$0.6377 &4.7438$\pm$0.4939 &0.8241$\pm$0.0799 &0.8972$\pm$0.0109 \\
     FusionNet &6.4257$\pm$0.8602 &5.1363$\pm$0.5151 &0.7961$\pm$0.0737 & 0.8746$\pm$0.0134\\
     LAGNet &6.9545$\pm$0.4739 &5.3262$\pm$0.3185 &0.8054$\pm$0.0837 &0.9125$\pm$0.0101 \\
     DCFNet &5.6194$\pm$0.6039 &\ul{4.4887$\pm$0.3764} &\ul{0.8292$\pm$0.0815} &\ul{0.9154$\pm$0.0083} \\
     \hline
     DDRF(ours) &\textbf{5.3827$\pm$0.5737} &4.6712$\pm$0.4155 &0.8217$\pm$0.0777 &0.8993$\pm$0.0129 \\
     \hline
     Ideal value & \textbf{0} & \textbf{0} & \textbf{1} & \textbf{1}\\
     \hline
    \end{tabular}
    }
\end{table}

\begin{table}[!htbp]
\centering
\caption{Generalization ability comparisons on WV2 full-resolution dataset.}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|ccc}
\hline
method    & $D_\lambda$($\pm$ std) & $D_s$($\pm$ std)  & QNR($\pm$ std)    \\
\hline \hline
PNN       & 0.1484$\pm$0.0957      & 0.0771$\pm$0.0169 & 0.7869$\pm$0.0959 \\
PanNet    & 0.0317$\pm$0.0173      & 0.0191$\pm$0.0123 & 0.9500$\pm$0.0275 \\
DiCNN     & 0.1412$\pm$0.0661      & 0.1023$\pm$0.0195 & 0.7700$\pm$0.0505 \\
MSDCNN    & 0.0589$\pm$0.0421      & 0.0290$\pm$0.0138 & 0.9143$\pm$0.0516 \\
FusionNet & 0.0519$\pm$0.0292      & 0.0559$\pm$0.0146 & 0.8948$\pm$0.0187 \\
LAGConv   & 0.1302$\pm$0.0856      & 0.0547$\pm$0.0159 & 0.8229$\pm$0.0884 \\
DCFNet    & $\pm$                  & $\pm$             & $\pm$             \\
\hline
DDRF(ours) & \textbf{0.0313$\pm$0.0376} & \textbf{0.0312$\pm$0.0111} & \textbf{0.9388$\pm$0.0453} \\
\hline
\end{tabular}%
}
\end{table}

